Faithful and Efficient Explanations for Neural Networks via Neural Tangent Kernel Surrogate Models

A recent trend in explainable AI research has focused on surrogate modeling, where neural networks are approximated as simpler ML algorithms such as kernel machines. A second trend has been to utilize kernel functions in various explain-by-example or data attribution tasks. In this work, we combine these two trends to analyze approximate empirical neural tangent kernels (eNTK) for data attribution. Approximation is critical for eNTK analysis due to the high computational cost to compute the eNTK. We define new approximate eNTK and perform novel analysis on how well the resulting kernel machine surrogate models correlate with the underlying neural network. We introduce two new random projection variants of approximate eNTK which allow users to tune the time and memory complexity of their calculation. We conclude that kernel machines using approximate neural tangent kernel as the kernel function are effective surrogate models, with the introduced trace NTK the most consistent performer. Open source software allowing users to efficiently calculate kernel functions in the PyTorch framework is available (https://github.com/pnnl/projection\_ntk).

==> adversarial_experiment_details.tex <==
	\section{Adversarial Experiment Details}
    	We trained our models on the MNIST dataset. In order to avoid combinatorial considerations, we trained a classifier on just two classes-- we used 7's and 1's because these digits look similar. To attack the models, we considered $\ell_\infty$ perturbations, computed using the projective gradient descent algorithm with 7 steps (PGD-7). We did not restrict pixel values of the attacked images to the interval $[0,1]$. See \cite{madry2019deep} for more information on using the PGD algorithm in an adversarial context. the However, in the PGD algorithm, attacking the SVM trained with the NTK involves computing second derivatives of the neural net. Due to this consideration, using ReLUs as neurons in this experiment was impractical-- the second derivative of a piecewise linear function at any point is either zero or non-existent. Hence the nets are constructed from sigmoid neurons.
    
		The model architecture was 3 fully connected layers of 100 neurons. The models were trained for 100 epochs and with learning rate $10^{-4}$ with AdamW optimizer and minibatches of size 64 using the standard SGD optimizer in PyTorch on the cross-entropy loss. The error bars in both Figures \ref{fig:white} and \ref{fig:grey} are for 10 neural nets.
